Real-Time Coupled Cluster Theory with Approximate Triples

In order to explore the effects of high levels of electron correlation on the real-time coupled cluster formalism and algorithmic behavior, we introduce a time-dependent implementation of the CC3 singles, doubles and approximate triples method. We demonstrate the validity of our derivation and implementation using specific applications of frequency-dependent properties. Terms with triples are calculated and added to the existing CCSD equations, giving the method a nominal $\textit{O}(N^{7})$ scaling. We also use a graphics processing unit (GPU) accelerated implementation to reduce the computational cost, which we find can speed up the calculation by up to a factor of 17 for test cases of water clusters. In addition, we compare the impact of using single-precision arithmetic compared to conventional double-precision arithmetic. We find no significant difference in polarizabilities and optical-rotation tensor results, but a somewhat larger error for first hyperpolarizabilities. Compared to linear response (LR) CC3 results, the percentage errors of RT-CC3 polarizabilities and RT-CC3 first hyperpolarizabilities are under 0.1% and 1%, respectively, for a water-molecule test case in a double-zeta basis set. Furthermore, we compare the dynamic polarizabilities obtained using RT-CC3, RT-CCSD, and time-dependent nonorthogonal orbital-optimized coupled cluster doubles (TDNOCCD), in order to examine the performance of RT-CC3 and the orbital-optimization effect using a set of ten-electron systems.

==> eoms.tex <==
\section*{Appendix---notes (TBP)}

Assuming a closed-shell spin-restricted reference determinant, the Hamiltonian can be written in the canonical basis as
\begin{align}
  &\hat{H}(t) = \hat{F} + \hat{U} + \hat{V}(t), \\
  &\hat{F} = \sum_p \epsilon_p \hat{E}_{pp}, \\
  &\hat{U} = \hat{H}(t) - \hat{V}(t) - \hat{F}.
\end{align}
The $T_1$-transformed Hamiltonian is (dropping the reference to time dependence for convenience):
\begin{equation}
  H = \mathrm{e}^{-\hat{T}_1} \hat{H} \mathrm{e}^{\hat{T}_1} = F + U + V,
\end{equation}
where $F = \exp(-\hat{T}_1) \hat{F} \exp(\hat{T}_1)$ and analogously for $U$ and $V$.
We assume that $\hat{V}$ is a one-electron operator.

The time-dependent CCSDT Lagrangian can be written as
\begin{align}
  \mathcal{L}_\text{CCSDT} &= \lambda_0 \braket{\phi_0\vert H + [H,\hat{T}_2] \vert \phi_0} \nonumber \\
  &+ \braket{\phi_0 \vert \hat{\Lambda}_1 \left( H + [H,\hat{T}_2] + [H,\hat{T}_3] \right) \vert \phi_0} \nonumber \\
  &+ \braket{\phi_0 \vert \hat{\Lambda}_2 \left( H + [H,\hat{T}_2] + [H,\hat{T}_3] + \frac{1}{2} [[H,\hat{T}_2],\hat{T}_2] \right) \vert \phi_0}
  \nonumber \\
  &+ \braket{\phi_0 \vert \hat{\Lambda}_3 \left( [H,\hat{T}_2] + [H,\hat{T}_3] + \frac{1}{2} [[H,\hat{T}_2],\hat{T}_2] 
                                               + [[H,\hat{T}_2],\hat{T}_3] \right) \vert \phi_0}
  \nonumber \\
  &- \mathrm{i} \lambda_0 \dot{\tau}_0 - \mathrm{i} \sum_{\mu_1} \lambda_{\mu_1} \dot{\tau}_{\mu_1}
  - \mathrm{i} \sum_{\mu_2} \lambda_{\mu_2} \dot{\tau}_{\mu_2} - \mathrm{i} \sum_{\mu_3} \lambda_{\mu_3} \dot{\tau}_{\mu_3},
\end{align}
To obtain the CC3 Lagrangian we now apply the following rules regarding order in the fluctuation potential $\hat{U}$,
\begin{alignat*}{2}
    &\text{Order}\ 0: &\qquad & \hat{F}, \hat{V}, \hat{T}_1, \hat{\Lambda}_1 \\
    &\text{Order}\ 1: &\qquad & \hat{U}, \hat{T}_2, \hat{\Lambda}_2 \\
    &\text{Order}\ 2: &\qquad & \hat{T}_3, \hat{\Lambda}_3
\end{alignat*}
and \emph{neglect all terms above fourth order in the CCSDT Lagrangian}:
\begin{align}
  \mathcal{L}_\text{CC3} &= \lambda_0 \braket{\phi_0\vert H + [H,\hat{T}_2] \vert \phi_0} \nonumber \\
  &+ \braket{\phi_0 \vert \hat{\Lambda}_1 \left( H + [H,\hat{T}_2] + [H,\hat{T}_3] \right) \vert \phi_0} \nonumber \\
  &+ \braket{\phi_0 \vert \hat{\Lambda}_2 \left( H + [H,\hat{T}_2] + [H,\hat{T}_3] + \frac{1}{2} [[H,\hat{T}_2],\hat{T}_2] \right) \vert \phi_0}
  \nonumber \\
  &+ \braket{\phi_0 \vert \hat{\Lambda}_3 \left( [H,\hat{T}_2] + [F+V,\hat{T}_3] + \frac{1}{2} [[V,\hat{T}_2],\hat{T}_2] \right) \vert \phi_0}
  \nonumber \\
  &- \mathrm{i} \lambda_0 \dot{\tau}_0 - \mathrm{i} \sum_{\mu_1} \lambda_{\mu_1} \dot{\tau}_{\mu_1}
  - \mathrm{i} \sum_{\mu_2} \lambda_{\mu_2} \dot{\tau}_{\mu_2} - \mathrm{i} \sum_{\mu_3} \lambda_{\mu_3} \dot{\tau}_{\mu_3}.
\end{align}
The EOMs can now be obtained from the Euler-Lagrange equations
\begin{equation}
    \frac{\partial \mathcal{L}_\text{CC3}}{\partial z} - \frac{\mathrm{d}}{\mathrm{d} t} \frac{\partial \mathcal{L}_\text{CC3}}{\partial \dot{z}} = 0,
\end{equation}
where $z$ denotes the cluster amplitudes $\tau$ and $\lambda$.

Setting $z = \lambda_0$, we find
\begin{equation}
    \mathrm{i}\dot{\tau}_0 = \braket{\phi_0\vert H + [H,\hat{T}_2] \vert \phi_0}.
\end{equation}
Setting $z = \tau_0$, we find
\begin{equation}
    \dot{\lambda}_0 = 0,
\end{equation}
which means that we may choose $\lambda_0 = 1$.

The remaining $\tau$ equations read (obtained by setting $z=\lambda_{\mu_i},\ i=1,2,3$):
\begin{align}
    \mathrm{i} \dot{\tau}_{\mu_1} &=
    \braket{\phi_{\mu_1} \vert H + [H,\hat{T}_2] + [H,\hat{T}_3] \vert \phi_0}, \\
    \mathrm{i} \dot{\tau}_{\mu_2} &=
    \braket{\phi_{\mu_2} \vert H + [H,\hat{T}_2] + [H,\hat{T}_3] + \frac{1}{2} [[H,\hat{T}_2],\hat{T}_2] \vert \phi_0}, \\
    \mathrm{i} \dot{\tau}_{\mu_3} &=
    \braket{\phi_{\mu_3} \vert [H,\hat{T}_2] + [F+V,\hat{T}_3] + \frac{1}{2} [[V,\hat{T}_2],\hat{T}_2] \vert \phi_0},
\end{align}
and the $\lambda$ equations read (obtained by setting $z = \tau_{\mu_i},\ i=1,2,3$):
\begin{align}
    -\mathrm{i} \dot{\lambda}_{\mu_1} &= \braket{\phi_0\vert [H, \hat{X}_{\mu_1}] \vert \phi_0} \nonumber \\
    &+ \braket{\phi_0 \vert \hat{\Lambda}_1 \left( [H, \hat{X}_{\mu_1}] + [[H, \hat{X}_{\mu_1}],\hat{T}_2] \right) \vert \phi_0} \nonumber \\
    &+ \braket{\phi_0 \vert \hat{\Lambda}_2 \left( [H, \hat{X}_{\mu_1}] + [[H, \hat{X}_{\mu_1}],\hat{T}_2] 
                                                 + [[H, \hat{X}_{\mu_1}],\hat{T}_3] \right) \vert \phi_0} \nonumber \\
    &+ \braket{\phi_0 \vert \hat{\Lambda}_3 \left( [H, \hat{X}_{\mu_1}],\hat{T}_2] + [[V, \hat{X}_{\mu_1}],\hat{T}_3] \right) \vert \phi_0},\\
    -\mathrm{i} \dot{\lambda}_{\mu_2} &=  \braket{\phi_0\vert [H,\hat{X}_{\mu_2}] \vert \phi_0} \nonumber \\
    &+ \braket{\phi_0 \vert \hat{\Lambda}_1 [H,\hat{X}_{\mu_2}] \vert \phi_0} \nonumber \\
    &+ \braket{\phi_0 \vert \hat{\Lambda}_2 \left( [H,\hat{X}_{\mu_2}] + [[H,\hat{X}_{\mu_2}],\hat{T}_2] \right) \vert \phi_0}
  \nonumber \\
    &+ \braket{\phi_0 \vert \hat{\Lambda}_3 \left( [H,\hat{X}_{\mu_2}] + [[V,\hat{X}_{\mu_2}],\hat{T}_2] \right) \vert \phi_0}, \\
    -\mathrm{i} \dot{\lambda}_{\mu_3} &=
    \braket{\phi_0 \vert \hat{\Lambda}_1 [H,\hat{X}_{\mu_3}] \vert \phi_0} \nonumber \\
    &+ \braket{\phi_0 \vert \hat{\Lambda}_2 [H,\hat{X}_{\mu_3}] \vert \phi_0}
  \nonumber \\
    &+ \braket{\phi_0 \vert \hat{\Lambda}_3 [F+V,\hat{X}_{\mu_3}] \vert \phi_0}.
\end{align}
Note that
\begin{equation}
    [F, \hat{T}_3] = [\hat{F}, \hat{T}_3] = \sum_{\mu_3} \epsilon_{\mu_3} \tau_{\mu_3} \hat{X}_{\mu_3}
\end{equation}

